Learning Vertex Representations for Bipartite Networks

Recent years have witnessed a widespread increase of interest in network representation learning (NRL). By far most research efforts have focused on NRL for homogeneous networks like social networks where vertices are of the same type, or heterogeneous networks like knowledge graphs where vertices (and/or edges) are of different types. There has been relatively little research dedicated to NRL for bipartite networks. Arguably, generic network embedding methods like node2vec and LINE can also be applied to learn vertex embeddings for bipartite networks by ignoring the vertex type information. However, these methods are suboptimal in doing so, since real-world bipartite networks concern the relationship between two types of entities, which usually exhibit different properties and patterns from other types of network data. For example, E-Commerce recommender systems need to capture the collaborative filtering patterns between customers and products, and search engines need to consider the matching signals between queries and webpages.

==> 3_method.tex <==
\section{Neural Factorization Machines}
\label{sec:method}
We first present the NFM model that unifies the strengths of FMs and neural networks for sparse data modelling.
We then discuss the learning procedure and how to employ some useful techniques in neural networks --- dropout and batch normalization ---  for NFM. 

\subsection{The NFM Model}
%The NFM model enhances FM by modeling higher-order and non-linear feature interactions under the neural network framework. 
Similar to factorization machine, NFM is a general machine learner working with any real valued feature vector.
Given a sparse vector $\textbf{x}\in \mathbb{R}^n$ as input, where a feature value $x_i = 0$ means the $i$-th feature does not exist in the instance, NFM estimates the target as:
\begin{equation}
	\hat{y}_{NFM}(\textbf{x}) = w_0 + \sum_{i=1}^n w_i x_i + f(\textbf{x}),
\end{equation}
where the first and second terms are the linear regression part similar to that for FM, which models global bias of data and weight of features. The third term $f(\textbf{x})$ is the core component of NFM for modelling feature interactions, which is a multi-layered feed-forward neural network as shown in Fig.~\ref{fig:nfm_model}. In what follows, we elaborate the design of $f(\textbf{x})$ layer by layer. \\\vspace{-5pt}

\textbf{Embedding Layer.} The embedding layer is a fully connected layer that projects each feature to a dense vector representation. Formally, let $\textbf{v}_i\in \mathbb{R}^k$ be the embedding vector for the $i$-th feature. After embedding, we obtain a set of embedding vectors $\mathcal{V}_x = \{x_1 \textbf{v}_1, ..., x_n \textbf{v}_n\}$ to represent the input feature vector $\textbf{x}$. 
Owing to sparse representation of $\textbf{x}$, we only need to include the embedding vectors for non-zero features, \ie $\mathcal{V}_x = \{x_i \textbf{v}_i \}$ where $x_i\neq 0$.
Note that we have rescaled an embedding vector by its input feature value, rather than simply an embedding table lookup, so as to account for the real valued features~\cite{FM}. 

\textbf{Bi-Interaction Layer.} We then feed the embedding set $\mathcal{V}_x$ into the Bi-Interaction layer, which is a pooling operation that converts a set of embedding vectors to one vector:
\begin{equation}
\label{eq:BI}
f_{BI}(\mathcal{V}_{x}) = \sum_{i=1}^n \sum_{j=i+1}^n x_i\textbf{v}_i\odot x_j\textbf{v}_j,
\end{equation}
where $\odot$ denotes the element-wise product of two vectors, that is, $(\textbf{v}_i \odot \textbf{v}_j)_k = v_{ik}v_{jk}$. 
Clearly, the output of Bi-Interaction pooling is a $k$-dimension vector that encodes the second-order interactions between features in the embedding space. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/nfm_model.pdf}
	\vspace{-5pt}
	\caption{Neural Factorization Machines model (the first-order linear regression part is not shown for clarity).}
	\vspace{-10pt}
	\label{fig:nfm_model}
\end{figure}

It is worth pointing out that our proposal of Bi-Interaction pooling does not introduce extra model parameter, and more importantly, it can be efficiently computed in linear time. 
This property is the same with average/max pooling and concatenation that are rather simple but commonly used in neural network  approaches~\cite{Wang:2015,He:WWW2017,DeepCross}.
To show the linear time complexity of evaluating Bi-Interaction pooling, we reformulate Equation~(\ref{eq:BI}) as:
\begin{equation}
\label{eq:BI2}
f_{BI}(\mathcal{V}_{x}) = \frac{1}{2} \left[( \sum_{i=1}^n x_i\textbf{v}_i)^2 - \sum_{i=1}^n (x_i\textbf{v}_i)^2 \right],
\end{equation}
where we use the symbol $\textbf{v}^2$ to denote $\textbf{v}\odot\textbf{v}$. By considering the sparsity of $\textbf{x}$, we can actually perform Bi-Interaction pooling in $O(k N_x)$ time, where $N_x$ denotes the number of non-zero entries in $\textbf{x}$. This is a very appealing property, meaning that the benefit of Bi-Interaction pooling in modelling pairwise feature interactions does not involve any additional cost. 

\textbf{Hidden Layers}. 
Above the Bi-Interaction pooling layer is a stack of fully connected layers, which are capable of learning higher-order interactions between features~\cite{DeepCross}. Formally, the definition of fully connected layers is as follows:
\begin{equation}
\begin{aligned}
	\textbf{z}_1 &= \sigma_1 (\textbf{W}_1 f_{BI}(\mathcal{V}_x) + \textbf{b}_1 ), \\
	\textbf{z}_2 &= \sigma_2 (\textbf{W}_2 \textbf{z}_1 + \textbf{b}_2), \\
	&\quad\quad ... ... \\
	\textbf{z}_L &= \sigma_L (\textbf{W}_L \textbf{z}_{L-1} + \textbf{b}_L),
\end{aligned}
\end{equation}
where $L$ denotes the number of hidden layers, $\textbf{W}_l$, $\textbf{b}_l$ and $\sigma_l$ denote the weight matrix, bias vector and activation function for the $l$-th layer, respectively. By specifying non-linear activation functions, such as sigmoid, hyperbolic tangent (tanh), and Rectifier (ReLU), we allow the model to learn higher-order feature interactions in a non-linear way. 
This is advantageous to existing methods for higher-order interaction learning, such as higher-Order FM~\cite{blondel2016higher} and Exponential Machines~\cite{EM}, which only support the learning of higher-order interactions in a linear way. 
As for the structure of fully connected layers (\ie size of each layer), one can freely choose tower~\cite{WideDeep,He:WWW2017}, constant~\cite{DeepCross}, and diamond~\cite{zhang2016deep}, among others. 

\textbf{Prediction Layer.} At last, the output vector of the last hidden layer $\textbf{z}_L$ is transformed to the final prediction score:
\begin{equation}
	f(\textbf{x}) = \textbf{h}^T \textbf{z}_L, 
\end{equation}
where vector $\textbf{h}$ denotes the neuron weights of the prediction layer. \\\vspace{-5pt}

\noindent To summarize, we give the formulation NFM's predictive model as:
\begin{equation}
\begin{aligned}
	\hat{y}_{NFM}(\textbf{x}) &= w_0 + \sum_{i=1}^n w_i x_i  \\
	&+ \textbf{h}^T \sigma_L(\textbf{W}_L(...\sigma_1(\textbf{W}_1 f_{BI}(\mathcal{V}_x) + \textbf{b}_1)  ... ) + \textbf{b}_L),
\end{aligned}
\end{equation}
with all model parameters $\Theta = \{w_0, \{w_i, \textbf{v}_i\}, \textbf{h}, \{\textbf{W}_l, \textbf{b}_l\} \}$. Compared to FM, the additional model parameters of NFM are mainly $\{\textbf{W}_l, \textbf{b}_l\}$, which are used for learning higher-order interactions between features. In remainder of this subsection, we first show how NFM generalizes FM and discuss the connection of NFM between existing deep learning methods; we then analyze the time complexity of evaluating NFM model. 

\subsubsection{\textbf{NFM Generalizes FM}} 
\label{ss:nfm_generalizes_fm}
FM is a shallow and linear model, which can be seen as a special case of NFM with no hidden layer. 
To show this, we set $L$ to zero and directly project the output of Bi-Interaction pooling to prediction score. 
We term this simplified model as NFM-0, which is formulated as:
\begin{equation}
\begin{aligned}
	\hat{y}_{NFM-0} &= w_0 + \sum_{i=1}^n w_i x_i + \textbf{h}^T \sum_{i=1}^n \sum_{j=i+1}^n x_i\textbf{v}_i\odot x_j\textbf{v}_j \\
	& = w_0 + \sum_{i=1}^n w_i x_i + \sum_{i=1}^n \sum_{j=i+1}^n \sum_{f=1}^k h_f v_{if} v_{jf}\cdot x_i x_j.
\end{aligned}
\end{equation}
As can be seen, by fixing $\textbf{h}$ to a constant vector of $(1,...,1)$, we can exactly recover the FM model\footnote{Note that for NFM-0, a trainable $\textbf{h}$ can not improve the expressiveness of FM, since its impact on prediction can be absorbed into feature embeddings.}. 

It is worth pointing out that, to our knowledge, this is the first time FM has been expressed under the neural network framework.
While a recent work by Blondel \etal~\cite{blondel2016polynomial} has unified FM and Polynomial network via kernelization, their kernel view of FM only provides a new training algorithm and does not provide insight for improving the FM model.
Our new view of FM is highly instructive and provides more insight for improving FM. 
Particularly, we allow the use of various neural network techniques on FM to improve its learning and generalization ability.
For example, we can use dropout~\cite{srivastava2014dropout} --- a well-known technique in deep learning community to prevent overfitting --- on the Bi-Interaction layer as a way to regularize FM, which we find can be even more effective than the conventional $L_2$ regularization (see Fig.~\ref{fig:dropout_reg} of Section~\ref{sec:experiments}).

\subsubsection{\textbf{Relation to Wide\&Deep and DeepCross}}
NFM has a similar multi-layered neural architecture with several existing deep learning solutions~\cite{WideDeep,DeepCross,He:WWW2017}. 
The key difference is in the Bi-Interaction pooling component, which is uniquely used in NFM. 
Specifically, if we replace the Bi-Interaction pooling with concatenation and apply a tower-structure MLP (or residual units~\cite{cvpr16best}) to hidden layers, we can recover the Wide\&Deep (or DeepCross) model.
An obvious limitation of the concatenation operation is that it does not account for any interaction between features. 
As such, these deep learning approaches have to rely entirely on the following deep layers to learn meaningful feature interactions, which unfortunately can be difficult to train in practice (\cf Section~\ref{ss:difficulty_dnn}). 
Our use of Bi-Interaction pooling captures second-order feature interactions in the low level, which is more informative than the concatenation operation. 
This greatly facilitates the subsequent hidden layers of NFM to learn useful higher-order feature interactions in a much easier way. 

\subsubsection{\textbf{Time Complexity Analysis}}
\label{ss:time_complexity}
We have shown in Equation~(\ref{eq:BI2}) that Bi-Interaction pooling can be efficiently computed in $O(k N_x)$ time, which is the same as FM. Then the additional costs are caused by the hidden layers. 
For hidden layer $l$, the matrix-vector multiplication is the main operation which can be done in $O(d_{l-1} d_l)$, where $d_l$ denotes the dimension of the $l$-th hidden layer and $d_0=k$. The prediction layer only involves inner product of two vectors, for which the complexity is $O(d_L)$. 
As such, the overall time complexity for evaluating a NFM model is $O(k N_x + \sum_{l=1}^L d_{l-1}d_l )$, which is the same as that of Wide\&Deep and DeepCross. 

\subsection{Learning}
NFM can be applied to a variety of prediction tasks, including regression, classification and ranking. 
To estimate model parameters of NFM, we need to specify an objective function to optimize. 
For regression, a commonly used objective function is the squared loss:
\begin{equation}
\label{eq:squared_loss}
	L_{reg} = \sum_{\textbf{x}\in \mathcal{X}} (\hat{y}(\textbf{x}) - y(\textbf{x}))^2,
\end{equation}
where $\mathcal{X}$ denotes the set of instances for training, and $y(\textbf{x})$ denotes the target of instance $\textbf{x}$. The regularization terms are optional and omitted here, since we found that some techniques in neural network modelling such as dropout can well prevent NFM from overfitting. 
For classification task, we can optimize the hinge loss or log loss~\cite{He:WWW2017}. For ranking task, we can optimize pairwise personalized ranking loss~\cite{BPR,silkroad} or contrastive max-margin loss~\cite{zhang2013attribute}. 
%Due to space limitation, we do not elaborate on the choices of objective functions here. 
In this work, we focus on the regression task and optimize the squared loss of Equation~(\ref{eq:squared_loss}). The optimization for ranking/classification tasks can be done in the same way. 

Stochastic gradient descent (SGD) is a universal solver for optimizing neural network models. 
It iteratively updates the parameters until convergence. In each time, it randomly selects a training instance $\textbf{x}$, updating each model parameter towards the direction of its negative gradient:
\begin{equation}
	\theta = \theta - \eta\cdot 2 (\hat{y}(\textbf{x}) - y(\textbf{x})) \frac{d \hat{y}(\textbf{x})}{d \theta},
\end{equation}
where $\theta\in \Theta$ is a trainable model parameter, and $\eta>0$ is the learning rate that controls the step size of gradient descent. 
As NFM is a multi-layered neural network model, the gradient of $\hat{y}(\textbf{x})$ \wrt to each model parameter can be derived using the chain rule. 
Here we give only the differentiation of the Bi-Interaction pooling layer, since other layers are just standard operations in neural network modelling and have been widely implemented in ML toolkits like TensorFlow and Keras.
\begin{equation}
	\frac{d f_{BI}(\mathcal{V}_{x})}{d \textbf{v}_i} = (\sum_{j=1}^n x_j \textbf{v}_j) x_i - x_i^2 \textbf{v}_i =  \sum_{j=1, j\neq i}^n x_i x_j \textbf{v}_j.
\end{equation} 
As such, for end-to-end neural methods, upon plugging in the Bi-Interaction pooling layer, they can still be learned end-to-end.
To leverage the vectorization and parallelism speedup of modern computing platforms, mini-batch SGD is more widely used in practice, which samples a batch of training instances and updates model parameters based on the batch.
In our implementation, we use mini-batch Adagrad~\cite{Adagrad} as the optimizer, rather than the vanilla SGD. Its main advantage is that the learning rate can be self adapted during the training phase, which eases the pain of choosing a proper learning rate and leads to faster convergence than the vanilla SGD. 

\subsubsection{\textbf{Dropout}} 
While neural network models have strong representation ability, they are also easy to overfit the training data. Dropout~\cite{srivastava2014dropout} is a regularization technique for neural networks to prevent overfitting. The idea is to randomly drop neurons (along with their connections) of the neural network during training. That is, in each parameter update, only part of the model parameters that contributes to the prediction of $\hat{y}(\textbf{x})$ will be updated. 
Through this process, it can prevent complex co-adaptations of neurons on training data. 
It is important to note that in the testing phase, dropout must be disabled and the whole network is used for estimating $\hat{y}(\textbf{x})$. As such, dropout can also be seen as performing model averaging with smaller neural networks~\cite{srivastava2014dropout}. 

In NFM, to avoid feature embeddings co-adapt to each other and overfit the data, we propose to adopt dropout on the Bi-Interaction layer. Specifically, after obtaining $f_{BI}(\mathcal{V}_{x})$ which is a $k$-dimensional vector of latent factors, we randomly drop $\rho$ percent of latent factors, where $\rho$ is termed as the dropout ratio. 
Since NFM with no hidden layer degrades to the FM model, it can be seen as a new way to regularize FM. 
Moreover, we also apply dropout on each hidden layer of NFM to prevent the learning of higher-order feature interactions from co-adaptations and overfitting. 

\subsubsection{\textbf{Batch Normalization}}
One difficulty of training multi-layered neural networks is caused by the fact of covariance shift~\cite{ioffe2015batch}. It means that the distribution of each layer's inputs changes during training, as the parameters of the previous layers change.
As a result, the later layer needs to adapt to these changes (which are often noisy) when updating its parameters, which adversely slows down the training. To address the problem, Ioffe and Szegedy~\cite{ioffe2015batch} proposed \textit{batch normalization} (BN), which normalizes layer inputs to a zero-mean unit-variance Gaussian distribution for each training mini-batch. It has been shown that BN leads to faster convergence and better performance in several computer vision tasks~\cite{cvpr16best,zhang2016play}.

Formally, let the input vector to a layer be $\textbf{x}_i\in \mathbb{R}^d$ and all input vectors to the layer of the mini-batch be $\mathcal{B}=\{\textbf{x}_i\}$, 
then BN normalizes $\textbf{x}_i$ as:
\begin{equation}
	BN(\textbf{x}_i) = \gamma\odot(\frac{\textbf{x}_i - \mu_B}{\sigma_B}) + \beta,
\end{equation}
where $\mu_B = \frac{1}{|\mathcal{B}|}\sum_{i\in \mathcal{B}} \textbf{x}_i$ denotes the mini-batch mean, $\sigma_B^2 = \frac{1}{|\mathcal{B}|}\sum_{i\in \mathcal{B}} (\textbf{x}_i - \mu_B)^2 $ denotes the mini-batch variance, and $\gamma$ and $\beta$ are trainable parameters (vectors) to scale and shift the normalized value to restore the representation power of the network. 
Note that in testing, BN also needs to be applied, where $\mu_B$ and $\sigma_B$ are estimated from the whole training data. 

In NFM, to avoid the update of feature embeddings changing the input distribution to hidden layers or prediction layer, we perform BN on the output of the Bi-Interaction pooling. For each successive hidden layer, the BN is also applied. 

%To summarize, we give the formulation of NFM's predictive model with both BN and dropout enabled as:
%\begin{equation}
%\begin{aligned}
%\hat{y}(\textbf{x}) &= w_0 + \sum_{i=1}^n w_i x_i + \textbf{h}^T \textbf{z}_L, \\
%\textbf{z}_l &= Dropout(\sigma_l(BN(\textbf{W}_l \textbf{z}_{l-1} + \textbf{b}_l ))), \quad l=1,...,L\\
%\textbf{z}_0 &= Dropout(BN (f_{BI}(\mathcal{V}_x)) ).
%\end{aligned}
%\end{equation}


==> abstract.tex <==
\begin{abstract}
Network embedding is an important method for embedding the large-scale general networks
into low-dimensional latent space, in which each vertex is represented by a vector.
%
These latent representations capture and preserve the network structure,
witch is useful for many mining tasks such as link predict, recommendation, visualization, and
node classification.
%
Network embedding approaches proposed recent years only consider the relationships between nodes belonging the same type,
but the relationships between different types of entities should also be modeled.
%
The bipartite network is a ubiquitous data structure modeling such relationship between two entity types:
for example, users and items, queries and webpages, users and advertises.
%
Obviously, it is impracticable to learn the representations of bipartite networks by using the general network
embedding methods directly, because the distinction of the two type nodes will be ignored.
%
With such cases, we propose a novel bipartite network embedding method named BiNE, which capture and preserve
both the implicit relationships between nodes of the same types and the  explicit information between
nodes involving different types.
%
We demonstrate the efficiency and effectiveness of BiNE by applying its embedding vectors into
personalized recommendation task.
%
Empirical experiments illustrate that our proposed model has promising performance and outperforms several
state-of-the-art approaches on real datasets.
\end{abstract}


%%
%% The code below should be generated by the tool at
%% http://dl.acm.org/ccs.cfm
%% Please copy and paste the code instead of the example below.
%%
%\begin{CCSXML}
%<ccs2012>
% <concept>
%  <concept_id>10010520.10010553.10010562</concept_id>
%  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%  <concept_significance>500</concept_significance>
% </concept>
% <concept>
%  <concept_id>10010520.10010575.10010755</concept_id>
%  <concept_desc>Computer systems organization~Redundancy</concept_desc>
%  <concept_significance>300</concept_significance>
% </concept>
% <concept>
%  <concept_id>10010520.10010553.10010554</concept_id>
%  <concept_desc>Computer systems organization~Robotics</concept_desc>
%  <concept_significance>100</concept_significance>
% </concept>
% <concept>
%  <concept_id>10003033.10003083.10003095</concept_id>
%  <concept_desc>Networks~Network reliability</concept_desc>
%  <concept_significance>100</concept_significance>
% </concept>
%</ccs2012>
%\end{CCSXML}
%
%\ccsdesc[500]{Computer systems organization~Embedded systems}
%\ccsdesc[300]{Computer systems organization~Redundancy}
%\ccsdesc{Computer systems organization~Robotics}
%\ccsdesc[100]{Networks~Network reliability}
%
%
%%
%% End generated code
%%
%
%%
%%  Use this command to print the description
%%
%\printccsdesc

% We no longer use \terms command
%\terms{Theory}

\keywords{Bipartite network embedding; scalability; random walk; recommendation}

